Mapping stellar surfaces III: An Efficient, Scalable, and Open-Source Doppler Imaging Model

The study of stellar surfaces can reveal information about the chemical composition, interior structure, and magnetic properties of stars. It is also critical to the detection and characterization of extrasolar planets, in particular those targeted in extreme precision radial velocity (EPRV) searches, which must contend with stellar variability that is often orders of magnitude stronger than the planetary signal. One of the most successful methods to map the surfaces of stars is Doppler imaging, in which the presence of inhomogeneities is inferred from subtle line shape changes in high resolution stellar spectra. In this paper, we present a novel, efficient, and closed-form solution to the problem of Doppler imaging of stellar surfaces. Our model explicitly allows for incomplete knowledge of the local (rest frame) stellar spectrum, allowing one to learn differences from spectral templates while simultaneously mapping the stellar surface. It therefore works on blended lines, regions of the spectrum where line formation mechanisms are not well understood, or stars whose spots have intrinsically different spectra from the rest of the photosphere. We implement the model within the open source starry framework, making it fast, differentiable, and easy to use in both optimization and posterior inference settings. As a proof-of-concept, we use our model to infer the surface map of the brown dwarf WISE 1049-5319B, finding close agreement with the solution of Crossfield et al. (2014). We also discuss Doppler imaging in the context of EPRV studies and describe an interpretable spectral-temporal Gaussian process for stellar spectral variability that we expect will be important for EPRV exoplanet searches.

==> xstring.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "xstring"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\xstringname               {xstring}                             %
\def\xstringversion              {1.83}                              %
%                                                                    %
\def\xstringdate              {2019/02/06}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea                                   %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
% Package URL: https://www.ctan.org/pkg/xstring                      %
% Bug tracker: https://framagit.org/unbonpetit/xstring/issues        %
% Repository : https://framagit.org/unbonpetit/xstring/tree/master   %
% Copyright  : Christian Tellechea 2008-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) xstring.tex                                        %
%              2) xstring.sty                                        %
%              3) xstring-fr.tex                                     %
%              4) xstring-fr.pdf                                     %
%              5) xstring-en.tex                                     %
%              6) xstring-en.pdf                                     %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\usepackage\else
	\immediate\write-1 {Package: xstring \xstringdate\space v\xstringversion\space String manipulations (CT)}%
\fi
\newcount\integerpart
\newcount\decimalpart% compteurs utilis?s par xstring

\edef\restorexstringcatcode{\catcode\number`\_ =\number\catcode`\_\relax}
\catcode`\_=11

\long\def\xs_execfirst#1#2{#1}
\long\def\xs_execsecond#1#2{#2}
\long\def\xs_gobarg#1{}
\expandafter\def\expandafter\xs_gobspace\space{}
\def\xs_deftok#1#2{\let#1= #2\relax}\xs_deftok\xs_sptoken{ }
\long\def\xs_ifnxttok#1#2#3{\xs_deftok\xs_toksmatch{#1}\def\__truecode{#2}\def\__falsecode{#3}\xs_ifnxttok_a}
\def\xs_ifnxttok_a{\futurelet\__futurtok\xs_ifnxttok_b}
\def\xs_ifnxttok_b{%
	\xs_ifx{\__futurtok\xs_sptoken}
	{\afterassignment\xs_ifnxttok_a\let\__futurtok= }
	{\xs_ifx{\__futurtok\xs_toksmatch}\__truecode\__falsecode}%
}
\def\xs_ifstar#1{\xs_ifnxttok*{\xs_execfirst{#1}}}
\long\def\xs_testopt#1#2{\xs_ifnxttok[{#1}{#1[{#2}]}}
\long\def\xs_exparg#1#2{\expandafter\xs_exparg_a\expandafter{#2}{#1}}%
\long\def\xs_exparg_a#1#2{#2{#1}}
\long\def\xs_exptwoargs#1#2#3{\xs_exparg{\xs_exparg{#1}{#2}}{#3}}
\long\def\xs_eearg#1#2{\xs_exparg{\xs_exparg{#1}}{#2}}
\long\def\xs_edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\long\def\xs_addtomacro#1#2{\xs_exparg{\def#1}{#1#2}}
\long\def\xs_eaddtomacro#1#2{\xs_exparg{\xs_addtomacro#1}{#2}}
\long\def\xs_eeaddtomacro#1#2{\xs_exparg{\xs_eaddtomacro#1}{#2}}
\long\def\xs_endgroup_eaddtomacro#1#2{\xs_exparg{\endgroup\xs_addtomacro#1}{#2}}
\long\def\xs_beforespace#1 #2\_nil{#1}
\long\def\xs_afterspace#1 #2\_nil{#2}
\long\def\xs_gobtonil#1\_nil{}
\long\def\xs_gobtobrace#1#{}
\long\def\xs_ifx#1{\ifx#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\def\xs_ifnum#1{\ifnum#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\long\def\xs_ifempty#1{\expandafter\xs_ifx\expandafter{\expandafter\relax\detokenize{#1}\relax}}

\def\xs_toks_toverb{% lit 1 argument et le transforme en verb
\begingroup
\def\do##1{\catcode`##112 }%
\dospecials
\obeyspaces
\xs_read_verb
}

\def\setverbdelim#1{% d?finit quel est le d?limiteur de verb
\xs_exparg\xs_ifempty{\xs_gobarg#1}%
{}
{\errmessage{Package xstring Warning: verb delimiter "\detokenize{#1}" is not a single token}}%
\def\xs_read_verb##1#1##2#1{\endgroup\xs_assign_verb{##2}}% on appelle l'ex?cution de fin
}

% Assigne l'argument entre d?limiteur verb dans la sc #1
\def\verbtocs#1{%
\def\xs_assign_verb##1{\def#1{##1}}%
\xs_toks_toverb
}

\begingroup
\catcode0 3 \gdef\xs_twozeroschars{^^00}%
\catcode0 7 \xdef\xs_twozeroschars{\xs_twozeroschars^^00}%
\endgroup

\edef\xs_reserved_A{\long\def\noexpand\xs_assigntokenizeresult##1\xs_twozeroschars}
\xs_reserved_A#2{\endgroup\xs_exparg{\def#2}{\xs_gobarg#1}}

\def\tokenize#1#2{%
	\begingroup
	\xs_def\xs_reserved_A{#2}% on d?veloppe en accord avec \fullexpandarg ou \noexpandarg
	\everyeof\expandafter{\xs_twozeroschars#1}%
	\endlinechar-1
	\expandafter\xs_assigntokenizeresult\scantokens\expandafter{\expandafter\relax\xs_reserved_A}% on fait l'assignation
}%

\long\def\xs_assign_xstringresult#1#2{\xs_ifempty{#2}{#1}{\def#2{#1}}}

\def\xs_ldef{\long\def}
\def\xs_ledef{\long\edef}

\def\normalexpandarg{%
\let\xs_def\xs_ldef% on d?finit \xs_call avec \def
\def\xs_expand##1{\unexpanded\expandafter{##1}}%
}
\let\noexpandarg\normalexpandarg% synonyme

\def\expandarg{%
\let\xs_def\xs_ldef% on d?finit \xs_call avec \def
\def\xs_expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

\def\fullexpandarg{%
\let\xs_def\xs_ledef% on d?finit\xs_call avec \edef
\def\xs_expand##1{##1}% et on neutralise \xs_expand
}

\def\saveexpandmode{\let\xs_saved_def\xs_defarg\let\xs_saved_expand\xs_expand}
\def\restoreexpandmode{\let\xs_defarg\xs_saved_def\let\xs_expand\xs_saved_expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\xs_ifbeginwithbrace#1{%
	\csname xs_exec%
	\expandafter\xs_gobarg\string{%
		\expandafter\xs_gobarg\expandafter{\expandafter{\string#1}%
			\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_execfirst
			\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_gobarg
			\expandafter\expandafter\expandafter\xs_gobarg
			\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\xs_gobarg\string}%
	\xs_execsecond{first}{second}%
	\endcsname
}

% Cette macro interne prend la 1ere unit? syntaxique de #1 et assigne le r?sultat ? #2
\long\def\xs_returnfirstsyntaxunit#1#2{%
	\let\xs_toks\relax
	\xs_ifempty{#1}
	{\let#2\empty
	}
	{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
		{\def#2{ }}
		{\xs_ifbeginwithbrace{#1}
			{\def\xs_groupfound{\xs_exparg{\def#2}{\expandafter{#2}}\xs_gobtonil}% on met #2 dans des accolades et on finit
				\let\xs_toks\bgroup
				\afterassignment\xs_groupfound
				\def#2%
			}
			{\long\def\xs_assignfirstarg##1##2\_nil{\def#2{##1}}%
				\xs_assignfirstarg
			}%
			#1\_nil
		}%
	}%
}

\long\def\xs_removefirstsyntaxunit#1#2{%
	\xs_ifempty{#1}
	{\let#2\empty
	}
	{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
		{\xs_exparg\xs_ifbeginwithbrace{\xs_gobspace#1}
			{\xs_exparg{\def#2}{\xs_gobtobrace#1}}%
			{\xs_exparg{\def#2}{\xs_afterspace#1\_nil}}%
		}%
		{\xs_exparg{\def#2}{\xs_gobarg#1}}%
	}%
}

% Cette macro interne est utilis?e dans les macros ?toil?es pour :
% 1) d?velopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci ? l'aide de la macro \xs_def
% 2) Ensuite, on d?tokenize ce d?veloppement de fa?on n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\xs_expand_and_detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\xs_expand#1}% on d?veloppe #2 selon le mode de d?veloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d?tokenize et on assigne ? #1
}

\long\def\xs_expand_and_assign#1#2{\xs_def#1{#2}}% on d?veloppe #2 selon \fullexpandarg ou \normalexpandarg

\def\xs_arglist{0########1########2########3########4########5########6########7########8########9}

% \xs_assign_args{3} met dans la sc \xs_myarg les tokens "####1####2####3"
\def\xs_assign_args#1{\def\xs_assign_args_i0##1#1##2\_nil{\def\xs_myarg{##1#1}}\expandafter\xs_assign_args_i\xs_arglist\_nil}

% \xs_assign_opt_args{3} met dans la sc \xs_myarg les tokens "[####1]####2####3####4"
\def\xs_assign_opt_args#1{\xs_exparg\xs_assign_opt_args_i{\number\numexpr#1+1}}
\def\xs_assign_opt_args_i#1{\def\xs_assign_opt_args_ii0##11##2#1##3\_nil{\def\xs_myarg{[##11]##2#1}}\expandafter\xs_assign_opt_args_ii\xs_arglist\_nil}

% \xs_assign_one_arg{3} met dans la sc \xs_myarg les tokens "####3"
\def\xs_assign_one_arg#1{\xs_exparg\xs_assign_one_arg_i{\number\numexpr#1-1}{#1}}
\def\xs_assign_one_arg_i#1#2{\def\xs_assign_one_arg_ii##1#1##2#2##3\_nil{\def\xs_myarg{##2#2}}\expandafter\xs_assign_one_arg_ii\xs_arglist\_nil}

% #1 : num?ro du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num?ro de l'argument devant ?tre d?tokenis? si ?toile
\def\xs_buildlines#1#2#3#4{%
\let\xs_newlines\empty
\let\xs_newargs\empty
\def\xs_buildlines_i##1{%
\xs_exparg\xs_assign_one_arg{\number\numexpr##1+#1-1}%
\edef\xs_reserved_B{\noexpand\xs_expand\csname xs_arg_\romannumeral\numexpr##1\endcsname}%
\xs_ifnum{##1=1 }% si c'est le premier argument
{\xs_ifempty{#3}%
	{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
		\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
	}% et s'il y a un argument optionnel alors, on met des crochets
	{\xs_eaddtomacro\xs_newargs{\expandafter[\xs_reserved_B]}%
		\def\xs_reserved_B{xs_def}% ne pas d?tok?niser l'argument optionnel grace au \xs_def
	}%
}
{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
	\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
}%
\edef\xs_newlines{\unexpanded\expandafter{\xs_newlines}\expandafter\noexpand\csname\xs_reserved_B\endcsname\expandafter\noexpand\csname xs_arg_\romannumeral\numexpr##1\endcsname{\xs_myarg}}%
\xs_ifnum{##1<#2 }
{\xs_exparg\xs_buildlines_i{\number\numexpr##1+1}}
{}%
}%
\xs_buildlines_i1%
}

\def\xs_newmacro{%
	\xs_ifstar
	{\let\xs_reserved_D\empty\xs_newmacro_}
	{\let\xs_reserved_D\relax\xs_newmacro_0}%
}

% #1 : dernier num?ro de l'argument devant ?tre d?tokenis?
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\xs_newmacro_#1#2#3#4#5{%
	\edef\xs_reserved_A{xs_\expandafter\xs_gobarg\string#2}%
	\edef\xs_reserved_C{\expandafter\noexpand\csname\xs_reserved_A _\ifx\empty#3\empty _\fi\endcsname}%
	\edef\xs_reserved_B{%
		\long
		\ifx\empty\xs_reserved_D
			\def\noexpand#2{\noexpand\xs_ifstar
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_detokenize\expandafter\noexpand\xs_reserved_C}%
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
		\fi
		\ifx\empty#3\empty
		\else
			\def\expandafter\noexpand\xs_reserved_C{%
				\noexpand\xs_testopt{\expandafter\noexpand\csname\xs_reserved_A __\endcsname}{\ifx\xs_def\xs_ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \xs_reserved_B ? Il d?finit :
	% si #3 est vide : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM__}{\let\xs_assign\xs_expand_and_assign\xs_NOM__}}
	% si #3 existe   : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM_}{\let\xs_assign\xs_expand_and_assign\xs_NOM_}}
	%                  \xs_NOM_{\xs_testopt{\xs_NOM__}{#3}}}
	\xs_reserved_B
	\ifx\empty#3\empty
		\xs_buildlines1{#4}{#3}{#1}%
		\xs_assign_args{#4}%
	\else
		\xs_exparg{\xs_buildlines1}{\number\numexpr#4+1}{#3}{#1}%
		\xs_assign_opt_args{#4}%
	\fi
	\edef\xs_reserved_B{\def\expandafter\noexpand\csname\xs_reserved_A __\endcsname\xs_myarg}%
	\edef\xs_reserved_C{\unexpanded\expandafter{\xs_newlines}\edef\noexpand\xs_call}%
	\edef\xs_reserved_D{\noexpand\noexpand\expandafter\noexpand\csname\xs_reserved_A\endcsname\unexpanded\expandafter{\xs_newargs}}%
	\ifnum#5=1 \edef\xs_reserved_D{\noexpand\noexpand\noexpand\xs_testopt{\unexpanded\expandafter{\xs_reserved_D}}{}}\fi
	\xs_edefaddtomacro\xs_reserved_C{{\unexpanded\expandafter{\xs_reserved_D}}\noexpand\xs_call}%
	\xs_edefaddtomacro\xs_reserved_B{{\unexpanded\expandafter{\xs_reserved_C}}}%
	% Que fait \xs_reserved_B ? Il d?finit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\xs_NOM__[##2]##3##4##5{%
	%          \xs_def\xs_arg_i{##2}\xs_assign\xs_arg_ii{##3}\xs_assign\xs_arg_iii{##4}\xs_asign\xs_arg_iv{##5}%
	% si #5=0: \edef\xs_call{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}%
	% si #5=1: \edef\xs_call{\noexpand\xs_testopt{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_i}{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}{}}%
	%          \xs_call}
	\long\xs_reserved_B
	\edef\xs_reserved_B{%
		\def\expandafter\noexpand\csname\xs_reserved_A\endcsname
		\xs_myarg\ifnum#5=1 [\unexpanded{##}\number\numexpr\ifx\empty#3\empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \xs_reserved_B ? Il d?finit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \xs_NOM[##2]##3##4##5[##6]{#6}
	\long\xs_reserved_B
}

% macro g?n?rique qui lit \xs_reserved_C us par us
% 3 sous-routines sont appel?es ? des moments cl? :
% \xs_atendofgroup      (un groupe se finit, appel r?cursif)
% \xs_atbegingroup      (un groupe vient d'?tre ouvert)
% \xs_atnextsyntaxunit  (la future US n'est pas un groupe)
\def\xs_read_reserved_C{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\xs_atendofgroup
			\xs_read_reserved_C
		}%
	}
	{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exploregroups
		\xs_ifx{\bgroup\xs_toks}
		{\advance\integerpart1
			\begingroup
			\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
			\xs_calc_grouIP
			\def\xs_nestlevel{1}%
			\integerpart0
			\xs_atbegingroup
		}
		{\advance\decimalpart1
			\xs_atnextsyntaxunit
		}%
		\xs_read_reserved_C
	}%
}

% macro g?n?rique qui lit \xs_reserved_D en proc?dant ? des tests avec \IfBeginWith
% 1 sous-routine est appel?e :
% \xs_atoccurfound      (une occurrence a ?t? trouv?e)
\def\xs_read_reserved_D{%
	\xs_exparg\xs_ifempty{\xs_reserved_D}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_C}{{\unexpanded\expandafter{\xs_reserved_C}}}%
			}%
			\__temp
			\xs_read_reserved_D
		}%
	}%
	{\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_D\xs_reserved_E
		{\advance\decimalpart1
			\let\xs_reserved_D\xs_reserved_A
			\xs_atoccurfound
		}%
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_A
			\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
			\xs_exploregroups
			\xs_ifx{\bgroup\xs_toks}
			{\advance\integerpart1
				\begingroup
				\expandafter\def\expandafter\xs_reserved_D\xs_reserved_A
				\xs_calc_grouIP
				\let\xs_reserved_C\empty
				\def\xs_nestlevel{1}%
				\integerpart0
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
			}%
		}%
		\xs_read_reserved_D
	}%
}

\xs_newmacro\StrRemoveBraces{}{1}{1}{%
	\def\xs_reserved_C{#1}%
	\let\xs_reserved_B\empty
	\def\xs_nestlevel{0}%
	\xs_StrRemoveBraces_i
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#2}%
}

\def\xs_StrRemoveBraces_i{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\xs_endgroup_eaddtomacro\xs_reserved_B\xs_reserved_B
			\xs_StrRemoveBraces_i
		}%
	}
	{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_ifx{\bgroup\xs_toks}
		{\xs_ifx{\xs_exploregroups\relax}% on explore les groupes ?
			{\begingroup
				\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
				\def\xs_nestlevel{1}%
				\let\xs_reserved_B\empty
			}
			{\expandafter\xs_addtomacro\expandafter\xs_reserved_B\xs_reserved_A
			}%
		}
		{\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
		}%
		\xs_StrRemoveBraces_i
	}%
}

% \xs_cutafteroccur coupe l'argument #1 apr?s la #3?me occurrence de #2
% \xs_reserved_C : contient ce qui se trouve avant cette occurrence
% \xs_reserved_D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \xs_reserved_E : contient ce qui se trouve apr?s l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy?es sont vides
\long\def\xs_cutafteroccur#1#2#3{%
	\xs_ifnum{#3<1 }
	{\let\xs_reserved_C\empty\let\xs_reserved_E\empty\gdef\groupID{}}
	{\xs_cutafteroccur_i{#1}{#2}{#3}}%
}

\long\def\xs_cutafteroccur_i#1#2#3{%
	\def\xs_reserved_D{#1}\let\xs_reserved_C\empty\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
		{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
			}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% mange l'appel r?cursif \xs_read_reserved_D dans \xs_read_reserved_D
		}
		{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
		}%
	}%
	\xs_read_reserved_D
	\xs_ifnum{\decimalpart=\numexpr(#3)\relax}% occurrence trouv?e ?
	{\let\xs_reserved_E\xs_reserved_D
		\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
	}
	{\let\xs_reserved_C\empty
		\let\xs_reserved_E\empty
		\gdef\groupID{}%
	}%
}

\xs_newmacro*3\IfSubStr{1}{2}{0}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_ifempty{\xs_reserved_D}\xs_execsecond\xs_execfirst
}

\xs_newmacro*2\IfBeginWith{}{2}{0}{%
	\xs_ifempty{#2}%
	{\xs_execsecond}
	{\xs_IfBeginWith_i{#1}{#2}}%
}

\long\def\xs_IfBeginWith_i#1#2{%
	\xs_ifempty{#2}%
	{\xs_execfirst% #2 est vide, tous les tests sont pass?s avec succ?s : on renvoie #3
	}
	{\xs_ifempty{#1}%
		{\xs_execsecond% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
		}
		{\xs_returnfirstsyntaxunit{#2}\xs_reserved_B
			\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
			\xs_ifx{\xs_reserved_A\xs_reserved_B}% il y a ?galit?...
			{\xs_removefirstsyntaxunit{#2}\xs_reserved_B
				\xs_removefirstsyntaxunit{#1}\xs_reserved_A% on enl?ve les 1ere unit?s syntaxiques
				\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_A\xs_reserved_B
			}
			{\xs_execsecond
			}%
		}%
	}%
}

\xs_newmacro*2\IfEndWith{}{2}{0}{%
	\xs_ifempty{#2}%
	{\xs_execsecond
	}
	{\xs_StrCount{#1}{#2}[\xs_reserved_A]%
		\xs_ifnum{\xs_reserved_A=0 }
		{\xs_execsecond}
		{\xs_exparg\xs_ifempty{\xs_reserved_C}}%
	}%
}

\xs_newmacro*4\IfSubStrBefore{1,1}{3}{0}{\xs_IfSubStrBefore_i[#1]{#2}{#3}{#4}}

\def\xs_IfSubStrBefore_i[#1,#2]#3#4#5{%
	\def\xs_reserved_C{#3}%
	\xs_ifx{\xs_exploregroups\relax}% si on explore les groupes
	{\let\xs_reserved_B\empty
		\def\xs_nestlevel{0}%
		\xs_StrRemoveBraces_i% on retire les accolades
		\let\xs_reserved_C\xs_reserved_B
	}
	{}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#5}{#2}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#4}{#1}%
	\gdef\groupID{}%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	\xs_execsecond
	\xs_execfirst
}

\xs_newmacro*4\IfSubStrBehind{1,1}{3}{0}{\xs_IfSubStrBehind_i[#1]{#2}{#3}{#4}}
\long\def\xs_IfSubStrBehind_i[#1,#2]#3#4#5{\xs_IfSubStrBefore_i[#2,#1]{#3}{#5}{#4}}

\long\def\xs_formatnumber#1#2{%
	\xs_ifempty{#1}%
	{\def#2{0X}% si vide, renvoie 0X
	}
	{\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
		\def\xs_reserved_B{+}%
		\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\xs_removefirstsyntaxunit{#1}\xs_reserved_C
			\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\def#2{+0X}}
			{\xs_exparg{\def#2}{\expandafter+\expandafter0\xs_reserved_C}}%
		}
		{\def\xs_reserved_B{-}%
			\xs_ifx{\xs_reserved_A\xs_reserved_B}
			{\xs_removefirstsyntaxunit{#1}\xs_reserved_A
				\xs_exparg\xs_ifempty{\xs_reserved_A}%
				{\def#2{-0X}}%
				{\xs_exparg{\def#2}{\expandafter-\expandafter0\xs_reserved_A}}%
			}
			{\def#2{0#1}%
			}%
		}%
	}%
}

\xs_newmacro\IfInteger{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\let\xs_after_intpart\afterinteger
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
	{\xs_ifnum{\decimalpart=0 }
		{\xs_execfirst% partie d?cimale constitu?e de 0 --> seul cas o? on renvoie vrai
		}
		{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
			\xs_execsecond
		}%
	}
	{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
		\xs_execsecond
	}%
}

\xs_newmacro\IfDecimal{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
}

\begingroup\catcode`\@ 11
\long\gdef\xs_defafterinteger#1\relax\_nil{\def\@xs@afterinteger{#1}\let\afterinteger\@xs@afterinteger}
\long\gdef\xs_defafterdecimal#1\_nil{\def\@xs@afterdecimal{#1}\let\afterdecimal\@xs@afterinteger}
\endgroup

\def\xs_testdot{%
\let\xs_decsep\empty
\xs_ifnxttok.
{\def\xs_decsep{.}\xs_readdecimalpart}%
{\xs_testcomma}%
}

\def\xs_testcomma{%
	\xs_ifnxttok,
	{\def\xs_dessep{,}\xs_readdecimalpart}%
		{\xs_defafterdecimal}%
}

\long\def\xs_readdecimalpart#1#2\_nil{%
	\xs_ifempty{#2}
	{\def\xs_reserved_A{0X}}
	{\def\xs_reserved_A{0#2}}%
	\afterassignment\xs_defafterinteger\decimalpart\xs_reserved_A\relax\_nil
	\expandafter\xs_defafterdecimal\afterinteger\_nil
}

% test d'?galit? sur des chaines (et des chaines contenant des nombres)
\long\def\xs_IfStrEqFalse_i#1#2{\let\xs_reserved_A\xs_execsecond}
\long\def\xs_IfStrEqFalse_ii#1#2{% renvoie vrai si les 2 arg sont d?cimaux et s'ils sont ?gaux, faux sinon
	\xs_IfDecimal{#1}%
	{\xs_IfDecimal{#2}%
		{\ifdim#1pt=#2pt
				\let\xs_reserved_A\xs_execfirst
			\else
				\let\xs_reserved_A\xs_execsecond
			\fi% les 2 sont d?cimaux : on fait le test
		}%
		{\let\xs_reserved_A\xs_execsecond}% un seul est d?cimal
	}%
	{\let\xs_reserved_A\xs_execsecond}% #1 n'est pas d?cimal
}

\long\def\xs_TestEqual#1#2{% teste si les 2 arguments sont ?gaux
	\def\xs_reserved_A{#1}\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
	{\let\xs_reserved_A\xs_execfirst}% ?galit? parfaite des 2 chaines
	{\xs_reserved_D{#1}{#2}}%
	\xs_reserved_A
}

\xs_newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont ?gales
	\let\xs_reserved_D\xs_IfStrEqFalse_i
	\xs_TestEqual{#1}{#2}%
}

\xs_newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont ?gaux
	\let\xs_reserved_D\xs_IfStrEqFalse_ii
	\xs_TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\xs_ifstar
	{\xs_IfStringCase{\IfStrEq*}}%
	{\xs_IfStringCase\IfStrEq}%
}

\def\IfEqCase{%
	\xs_ifstar
	{\xs_IfStringCase{\IfEq*}}%
	{\xs_IfStringCase\IfEq}%
}

\long\def\xs_IfStringCase#1#2#3{% #1=macro avec ou sans ?toile  #2=argument ? tester  #3=liste des {<cas>}{code>}
	\long\def\xs_testcase##1##2##3\_nil{% lit les 2 premieres unit?s syntaxiques dans ##1 et ##2. Les autres dans ##3
		#1{#2}{##1}% compare
			{\xs_testopt{\xs_IfStringCase_ii{##2}}{}}% le test est positif, on ex?cute le code correspondant et on mange l'argument optionnel ## BUGfix dans 1.82
			{\xs_ifempty{##3}%
				{\xs_testopt{\xs_IfStringCase_i}{}}% s'il n'y a plus de cas, on ex?cute le code <autres cas> ## BUGfix dans 1.82
				{\xs_testcase##3\_nil}% sinon, on recommence avec ce qui reste
			}%
	}%
	\xs_testcase#3\_nil
}

\long\def\xs_IfStringCase_i[#1]{#1}
\long\def\xs_IfStringCase_ii#1[#2]{#1}

% Renvoie ce qui est ? gauche de l'occurence n?#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBefore{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#4}%
}

% Renvoie ce qui est ? droite de l'occurence n?#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBehind{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n?#1 et n?#2
% des chaines #4 et #5 dans la chaine #3
\xs_newmacro*4\StrBetween{1,1}{3}{1}{\xs_StrBetween_i[#1]{#2}{#3}{#4}[#5]}
\long\def\xs_StrBetween_i[#1,#2]#3#4#5[#6]{%
	\begingroup
	\noexploregroups
	\xs_cutafteroccur{#3}{#5}{#2}%
	\xs_exparg\xs_cutafteroccur{\xs_reserved_C}{#4}{#1}%
	\expandafter
	\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_E}{#6}%
	\gdef\groupID{}%
}

\def\exploregroups{\let\xs_exploregroups\relax}
\def\noexploregroups{\def\xs_exploregroups{\let\xs_toks\relax}}
\def\saveexploremode{\let\xs_saveexploremode\xs_exploregroups}
\def\restoreexploremode{\let\xs_exploregroups\xs_saveexploremode}

% Remplace les #1 premi?res occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\xs_newmacro\StrSubstitute{0}{3}{1}{%
	\def\xs_reserved_D{#2}\let\xs_reserved_C\empty\def\xs_reserved_E{#3}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{#1<1 }
		{\def\xs_reserved_A{#4}}
		{\xs_ifnum{\decimalpart>#1 }
			{\def\xs_reserved_A{#3}}
			{\def\xs_reserved_A{#4}}%
		}%
		\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
	}%
	\xs_ifempty{#3}%
	{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#5}%
	}
	{\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#5}%
	}%
}

% Supprime les #1 premi?res occurrences de #3 dans #2
\xs_newmacro\StrDel{0}{2}{1}{\xs_StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\xs_exitallgroups{\ifnum\xs_nestlevel>0 \endgroup\expandafter\xs_exitallgroups\fi}

% Compte combien d'unit?s syntaxiques contient la chaine #1 ?
\xs_newmacro\StrLen{}{1}{1}{%
	\def\xs_reserved_C{#1}\decimalpart0 \def\xs_nestlevel{0}\gdef\groupID{0}%
	\let\xs_atbegingroup\relax
	\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
	\let\xs_atnextsyntaxunit\relax
	\xs_read_reserved_C
	\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n?cessaire pour trouver une unit? syntaxique derri?re
\def\xs_continuetonext{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\ifnum\xs_nestlevel>0
			\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}% on concat?ne
			\expandafter\xs_continuetonext% on recommence
		\fi}
	{}%
}%

\def\xs_calc_grouIP{%
	\begingroup\def\xs_reserved_A{0}%
	\xs_ifx{\xs_reserved_A\groupID}% si on arrive du groupe de niveau 0
	{\endgroup\xdef\groupID{\number\integerpart}}% on met simplement le niveau
	{\endgroup\xs_eearg{\gdef\groupID}{\expandafter\groupID\expandafter,\number\integerpart}}%
}

% Cette macro coupe la chaine #1 apr?s l'unit? syntaxique n?#2
\def\StrSplit{%
	\xs_ifstar
	{\let\xs_reserved_E\xs_continuetonext\StrSplit_i}%
	{\let\xs_reserved_E\relax\StrSplit_i}%
}

\xs_newmacro\StrSplit_i{}{2}{0}{\xs_StrSplit_ii{#2}{#1}\xs_StrSplit_iii}

% Cette macro interne coupe la chaine #2 apr?s l'unit? syntaxique n?#1
% Le d?but est assign? dans \xs_reserved_B et la fin dans \xs_reserved_C
\long\def\xs_StrSplit_ii#1#2{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#2}\def\xs_reserved_D{#1}\gdef\groupID{}%
	\ifnum#1>0
		\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{%
			\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_B}{{\unexpanded\expandafter{\xs_reserved_B}}}%
			}%
			\__temp
		}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{%
			\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			\xs_ifnum{\decimalpart=\xs_reserved_D\relax}
			{\ifx\xs_reserved_C\empty\xs_reserved_E\fi
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_B}}\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}}%
				\expandafter\xs_exitallgroups\__temp
				\xs_gobarg% mange l'appel r?cursif \xs_read_reserved_C dans \xs_read_reserved_C
			}
			{}%
		}%
		\xs_read_reserved_C
	\fi
}

\def\xs_StrSplit_iii#1#2{\let#1\xs_reserved_B\let#2\xs_reserved_C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA re?oit ce qui se trouve avant la n ?me occurrence <motif> dans <texte>
% \macroB re?oit ce qui est apr?s cette n ?me occurrence
\xs_newmacro*3\StrCut{1}{2}{0}{%
	\xs_ifempty{#3}%
	{\gdef\groupID{}\let\xs_reserved_C\empty\let\xs_reserved_E\empty
	}
	{\xs_ifnum{#1<1 }
		{\xs_StrCut_ii{#2}{#3}1}
		{\xs_StrCut_ii{#2}{#3}{#1}}%
	}%
	\xs_StrCut_iii
}

\long\def\xs_StrCut_ii#1#2#3{%
	\let\xs_reserved_C\empty\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
		{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
			}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% stoppe la r?cursivit? dans \xs_read_reserved_D
		}
		{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
		}%
	}%
	\xs_read_reserved_D
	\let\xs_reserved_E\xs_reserved_D
	\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
}

\long\def\xs_StrCut_iii#1#2{\let#1\xs_reserved_C\let#2\xs_reserved_E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit?s syntaxiques aux positions compris !
\xs_newmacro\StrMid{}{3}{1}{%
	\begingroup
	\noexploregroups
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#3}{#1}%
	\edef\xs_reserved_C{\number\numexpr#2-1}%
	\let\xs_reserved_E\relax
	\xs_exptwoargs\xs_StrSplit_ii\xs_reserved_C\xs_reserved_B
	\expandafter\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_C}{#4}%
	\gdef\groupID{}%
}

% supprime #2 unit?s syntaxiques ? gauche dans la chaine #1
\xs_newmacro\StrGobbleLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

% extrait de #1 la chaine ? gauche de longueur #2
\xs_newmacro\StrLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% supprime #2 unit?s syntaxiques ? droite dans la chaine #1
\xs_newmacro\StrGobbleRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% renvoie #2 unit?s syntaxiques ? la droite de la chaine #1
\xs_newmacro\StrRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

\xs_newmacro\StrChar{}{2}{1}{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\ifnum#2>0
		\def\groupID{0}\def\xs_nestlevel{0}\integerpart0 \decimalpart0
		\let\xs_atbegingroup\relax
		\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
		\def\xs_atnextsyntaxunit{%
			\ifnum\decimalpart=\xs_reserved_D% la n i?me US est atteinte ?
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_A}}}% on capture l'US en cours qui est celle cherch?e
				\expandafter\xs_exitallgroups\__temp
				\expandafter\xs_gobarg% stoppe la r?cursivit? dans \xs_read_reserved_C
			\fi
		}%
		\xs_read_reserved_C
	\fi
	\xs_exparg\xs_ifempty{\xs_reserved_B}%
	{\gdef\groupID{}}
	{}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\xs_newmacro\StrCount{}{2}{1}{%
	\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}\let\xs_reserved_C\empty
	\xs_ifempty{#2}%
	{\xs_assign_xstringresult{0}{#3}%
	}
	{\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atoccurfound{\let\xs_reserved_C\empty\xs_read_reserved_D}%
		\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#3}%
	}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\xs_newmacro\StrPosition{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\let\xs_reserved_E\groupID
	\xs_ifx{\xs_reserved_C\xs_reserved_D}
	{\xs_assign_xstringresult{0}{#4}%
		\let\xs_reserved_E\empty
	}
	{\xs_exparg\xs_StrLen{\xs_reserved_C}[\xs_reserved_C]%
		\xs_exparg\xs_assign_xstringresult{\number\numexpr\xs_reserved_C+1}{#4}%
	}%
	\global\let\groupID\xs_reserved_E
}

\def\comparestrict{\def\xs_comparecoeff{1}}
\def\comparenormal{\def\xs_comparecoeff{0}}
\def\savecomparemode{\let\xs_saved_comparecoeff\xs_comparecoeff}
\def\restorecomparemode{\let\xs_comparecoeff\xs_saved_comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont ?gaux et renvoie la
% position de la premiere unit? syntaxiques diff?rente sinon
\xs_newmacro*2\StrCompare{}{2}{1}{%
	\def\xs_reserved_A{#1}%
	\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_B\xs_reserved_A}
	{\xs_assign_xstringresult{0}{#3}}
	{\xs_StrCompare_i{#1}{#2}{#3}}%
}

\long\def\xs_StrCompare_i#1#2#3{%
\def\xs_StrCompare_iii##1{%
\let\xs_reserved_A\empty
\xs_exparg\xs_ifempty{\xs_reserved_C}%
{\edef\xs_reserved_A{*\xs_comparecoeff}}%
{\xs_exparg\xs_ifempty{\xs_reserved_D}%
	{\edef\xs_reserved_A{*\xs_comparecoeff}}
	{}%
}%
\def\xs_next{\xs_exparg\xs_assign_xstringresult{\number\numexpr##1\xs_reserved_A\relax}{#3}}%
}%
\def\xs_StrCompare_ii##1{% ##1 est la position
\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_B
\xs_ifx{\xs_reserved_B\xs_reserved_A}
{\xs_exparg\xs_ifempty{\xs_reserved_A}%
	{\xs_StrCompare_iii{##1}% les 2 unit?s syntaxiques sont ?gales, on renvoie la position
	}
	{\def\xs_next{\xs_exparg\xs_StrCompare_ii{\number\numexpr##1+1}}% les 2 unit?s syntaxiques sont ?gales et non vides, on recommence
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
	}%
}% les 2 unit?s syntaxiques sont diff?rentes : on renvoie la position
{\xs_StrCompare_iii{##1}%
}%
\xs_next
}%
\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
\xs_StrCompare_ii1%
}

\xs_newmacro\StrFindGroup{}{2}{1}{%
	\def\xs_reserved_A{#2}\def\xs_reserved_B{0}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
	{\xs_assign_xstringresult{{#1}}{#3}}
	{\xs_StrFindGroup_i{#1}{#2}[#3]}%
}

\long\def\xs_StrFindGroup_i#1#2[#3]{%
	\def\xs_StrFindGroup_ii{%
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_assign_xstringresult{}{#3}% s'il ne reste plus rien, on renvoie vide
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_D
			\xs_ifx{\bgroup\xs_toks}% si la 1?re unit? syntaxique est un groupe explicite
			{\advance\decimalpart1 % on augmente le compteur
				\xs_ifnum{\decimalpart=\xs_reserved_A\relax}% on est au groupe cherch? lors de la profondeur courante ?
				{\xs_ifx{\empty\xs_reserved_B}% on est ? la profondeur maximale ?
					{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#3}}% on renvoie ce groupe
					{\xs_exparg{\expandafter\xs_StrFindGroup_i\xs_reserved_D}{\xs_reserved_B}[#3]}% on recommence avec ce groupe et les profondeurs de recherche restantes
				}
				{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
					\xs_StrFindGroup_ii
				}%
			}
			{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_StrFindGroup_ii
			}%
		}%
	}%
	\xs_extractgroupnumber{#2}\xs_reserved_A\xs_reserved_B
	\decimalpart0
	\xs_ifnum{\xs_reserved_A>0 }
	{\def\xs_reserved_C{#1}}
	{\let\xs_reserved_C\empty}%
	\xs_StrFindGroup_ii
}

\def\xs_extractgroupnumber#1#2#3{%
	\def\xs_extractgroupnumber_i##1,##2\_nil{\def#2{##1}\def#3{##2}}%
	\xs_extractgroupnumber_i#1,\_nil
	\ifx\empty#3\else\xs_extractgroupnumber_i#1\_nil\fi
}

\def\expandingroups{\let\xs_expandingroups\exploregroups}

\def\noexpandingroups{\let\xs_expandingroups\noexploregroups}

\def\StrExpand{\xs_testopt{\xs_StrExpand}{1}}
\long\def\xs_StrExpand[#1]#2#3{%
	\begingroup
	\xs_expandingroups
	\xs_ifnum{#1>0 }
	{\integerpart#1 \decimalpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{\xs_eeaddtomacro\xs_reserved_B{\xs_reserved_A}}%
		\def\xs_reserved_C{#2}%
		\xs_StrExpand_i{#1}% Appel de la macro r?cursive
	}
	{\def\xs_reserved_B{#2}%
	}
	\expandafter
	\endgroup
	\expandafter\def\expandafter#3\expandafter{\xs_reserved_B}%
	\gdef\groupID{}%
}

\long\def\xs_StrExpand_i#1{%
	\xs_ifnum{#1>0 }
	{\let\xs_reserved_B\empty
		\xs_read_reserved_C
		\let\xs_reserved_C\xs_reserved_B
		\def\xs_reserved_A{\xs_exparg\xs_StrExpand_i{\number\numexpr#1-1}}%
	}
	{\let\xs_reserved_A\relax
	}%
	\xs_reserved_A
}

\def\scancs{\xs_testopt{\xs_scancs}{1}}
\long\def\xs_scancs[#1]#2#3{%
	\xs_StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

\restorexstringcatcode

\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput

H I S T O R I Q U E
------------------------------------------------------------------------------
v1.0    4/7/2008 : - Package achev?.
7/7/2008 : - Package publi? sur CTAN.
------------------------------------------------------------------------------
v1.1    15/8/2008
- Le package ne n?cessite plus LaTeX et est d?sormais utilisable sous
Plain eTeX.
- Ajout des macros \IfInteger et \IfDecimal.
Pour cette derni?re, la partie enti?re et la partie d?cimale sont
r?cup?rables dans les compteurs \integerpart et \decimalpart. Ce
qu'il reste apr?s qu'un caract?re non attendu soit rencontr? est
dispo dans \xs_remainafterdecimal
- Correction d'un bug dans \tokenize :
suppression de l'expansion avec \normalexpandarg pour ?viter le bug
avec les lettres accentu?es dans l'exemple : \tokenize\aa{??}
- Am?lioration du code de la plupart des macros.
- ?criture d'une routine \xs_newmacro d?finissant les  macros.
- Suppression de tous les compteurs grace ? \numexpr.
- Nouvelles fonctionnalit?s internes dans :
\IfSubStr
ajout des chaines se trouvant avant et apr?s l'occurrence test?e
dans les sc \xs_behind_IfSubStr et \xs_before_IfSubStr
\StrCount
a) ajout de ce qui se trouve apr?s la derni?re occurrence dans la
sc \xs_StrCount_afterlastocccur
b) la macro ne d?pend plus d'aucune autre
------------------------------------------------------------------------------
v1.2    23/8/2008
- Am?lioration du code de \StrMid \StrGobbleLeft, \StrLeft,
\StrGobbleRight et \StrRight ? l'aide de la nouvelle macro
\xs_StrSplit_i
- Nouveau test \IfStrEq qui compare 2 chaines
- Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
contiennent un nombre)
- Correction d'un bug dans \xs_formatnumber. La macro n'envisageait pas le
cas o? son argument ?tait vide ce qui faiasait planter
\IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
------------------------------------------------------------------------------
v1.3    21/9/2008
- Am?lioration du code, mise en place de r?cursivit?s terminales dans
toutes les macros r?cursives, simplification de \xs_TestEqual en
utilisant \ifx
- Nouvelles macros \IfStrEqCase et \IfEqCase
Teste si une cha?ne est ?gale ? plusieurs chaines donn?es et
ex?cute un code sp?cifique
- Cr?ation de la macro publique \StrSplit
Coupe la chaine en 2 ? une position donn?e
- Nouvelle macro \StrCompare
Compare 2 cha?nes et renvoie la position du 1er caract?re diff?rent.
Renvoie 0 si elles sont ?gales.
------------------------------------------------------------------------------
v1.3a   29/9/2008
- Correction d'un bug : \expandafter#1
dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
nombre > 9 !
- R? ?criture de \xs_returnfirstsyntaxunit et \xs_gobarg qui
deviennent purement d?veloppables.
- R? ?criture de \StrLen
- Nouvelle macro interne \xs_cutafteroccur
Coupe la chaine apr?s la ni?me occurrence d'une sous chaine.
- Code am?lior? de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
\StrGobbleRight grace ? \xs_cutafteroccur
------------------------------------------------------------------------------
v1.4   4/11/2008
- xstring traite ses arguments par unit? syntaxique, et donc toutes les
macros internes ont ?t? r?-?crites ? cette fin.
- Le manuel a ?t? r?-?crit, rendu plus clair et mieux structur?.
- Nouvelle fonctionnalit? : \expandarg
le 1er lex?me de chaque argument est 1-d?velopp? avant que la
macro ne soit appel?e. Si un argument comporte plus qu'1 lex?me,
il faut passer par \scancs*[1] pour 1-d?velopper toutes les unit?s
syntaxiques.
- Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
d?faut dans \StrSubstitute et \StrDel
- Coh?rence dans les nom des s?quences de contr?les temporaires qui
sont d?sormais : \xs_reserved_A ? \xs_reserved_E
------------------------------------------------------------------------------
v1.4a  12/11/2008
- Correction d'un bug dans \xs_StrSplit dans le cas o? l'argument
num?rique est <1 : la 1ere coupure doit ?tre vide et le seconde doit
?tre ?gale ? l'argument.
------------------------------------------------------------------------------
v1.4b  16/11/2008
- Correction de 2 bugs dans \xs_returnfirstsyntaxunit
------------------------------------------------------------------------------
v1.5   31/12/2008
- Nouvelles fonctionnalit?s dans la recherche de groupes par un
identificateur caract?risant leur imbrication. Impl?mentation de :
1) \StrFindGroup
2) \groupID
- Ajout des nouvelles macros g?n?riques \xs_read_reserved_C et
\xs_read_reserved_D
- Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
que \truc contenait ?a{a}?.
- Correction d'un bug dans \xs_newmacro : l'argument optionnel ?tait
d?tok?nis? ? tort dans les macros ?toil?es.
- Dans \xs_newmacro, on doit choisir le num?ro du dernier argument devant
?tre d?tok?nis? dans le cas d'une macro ?toil?e (sachant que
l'argument optionnel ne l'est jamais)
------------------------------------------------------------------------------
v1.5a  09/2/2009
- Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
ind?pendante du mode d'exploration et dispose de ses propres commandes
d'exploration : \expandingroups et \noexpandingroups
- R?-?criture de \scancs, qui devient triviale puisque d?pendant de
\StrExpand. Il n'y a plus de version ?toil?e et d?sormais, \scancs
est sensible au mode d'exploration.
- Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
- Correction de bugs : mettre \let\xs_reserved_E\relax avant d'appeler
\xs_StrSplit_i
- Suppression des messages d'erreur, de warning et d'info. xstring devient
donc silencieux ;)
- Passage de 3 ? 2 compteurs
- Le manuel est d?sormais plus color?, en esp?rant qu'il sera un peu
plus agr?able ? lire !
------------------------------------------------------------------------------
v1.5b  13/3/2009
- Modification d'un grand nombre de macros de telle sorte que vraiment
n'importe quel code peut d?sormais ?tre plac? dans les arguments des
macros (comme par exemple des \if, \ifx ou autre, m?me sans leur \fi, ce
qui n'?tait pas possible jusqu'alors)
------------------------------------------------------------------------------
v1.5c  05/6/2009
- Correction d'un bug dans \IfBeginWith : il faut appeler
\xs_returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
non pas l'inverse pour que \xs_toks refl?te ce qui se trouve dans #1
- Correction d'un bug dans \xs_returnfirstsyntaxunit au cas o? #1 commence
par un espace : mettre \xs_toks ? 0
- Correction d'un bug dans \xs_returnfirstsyntaxunit :
\xs_returnfirstsyntaxunit{{}}\truc
faisait que \truc se d?veloppait en un espace.
- Correction d'un bug dans \xs_removefirstsyntaxunit o? le cas
\xs_removefirstsyntaxunit{ {b}}\truc
donnait \truc se d?veloppant en ?b? au lieu de ?{b}?.
------------------------------------------------------------------------------
v1.5d  28/3/2010
- Correction d'un bug dans \IfInteger : \afterinteger ne donnait pas le
bon r?sultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
- \xs_formatnumber ne detokenize plus ses arguments (que m'est-il pass?
par la t?te pour que je code un truc comme ca ?), et donc
\afterinteger et \xs_afterdecimal ont des tokens ayant le bon
catcode
------------------------------------------------------------------------------
v1.6  24/10/2012
- Correction d'un bug dans \xs_cutafteroccur au cas o? #3<1
- \IfDecimal ne \detokenize plus l'argument.
- Nouvelle version de \tokenize qui enlevait les accolades si son argument
?tait entre accolades
- Nouvelle macro \StrCut
- \xs_cutafteroccur_i ne produit plus d'espace ind?sirable si #3 ?tait
?valu? par \numexpr
------------------------------------------------------------------------------
v1.7  13/1/2013
- Correction d'un manque de rigueur dans les assignations concernant
\groupID : elles sont toutes globales d?sormais
- Les macros de xstring sont \long
------------------------------------------------------------------------------
v1.7a 28/2/2013
- Correction d'un espace parasite dans \xs_removefirstsyntaxunit
------------------------------------------------------------------------------
v1.7b 29/7/2013
- La date contenue dans \xstringdate est d?sormais conforme
------------------------------------------------------------------------------
v1.7c 13/10/2013
- les macros impliqu?es dans \IfStrCase et \IfStrEqCase sont d?sormais \long
------------------------------------------------------------------------------
v1.8  07/12/2018
- affectations globales supprim?es (sauf pour \groupID) afin de ne pas
surcharger la pile de sauvegarde
- nettoyage du code, corrections de lourdeurs et maladresses
------------------------------------------------------------------------------
v1.81 09/12/2018
- bug dans \IfInteger et \IfDecimal, la macro \xs_afterdecimal est ind?finie
et doit ?tre remplac?e par \afterdecimal
------------------------------------------------------------------------------
v1.82 01/02/2019
- \xs_testopt n'est pas longue et provoque un bug dans \xs_IfStrCase et
\xs_IfStrCase lorsque #1 contient \par : \xs_testopt reste courte et
\xs_IfStringCase a ?t? modifi?e pour que cela fonctionne.
------------------------------------------------------------------------------
v1.83 06/02/2019
- mauvaise approche et mauvais fix dans la v1.82 : \xs_testopt devient
longue, pas le choix (et donc aussi \xs_ifnxttok)

